Search for heavy particles decaying into top-quark pairs using lepton-plus-jets events in proton-proton collisions at $\sqrt{s} = 13$ TeV with the ATLAS detector

A search for new heavy particles that decay into top-quark pairs is performed using data collected from proton-proton collisions at a centre-of-mass energy of 13 TeV by the ATLAS detector at the Large Hadron Collider. The integrated luminosity of the data sample is 36.1 fb$^{-1}$. Events consistent with top-quark pair production are selected by requiring a single isolated charged lepton, missing transverse momentum and jet activity compatible with a hadronic top-quark decay. Jets identified as likely to contain $b$-hadrons are required to reduce the background from other Standard Model processes. The invariant mass spectrum of the candidate top-quark pairs is examined for excesses above the background expectation. No significant deviations from the Standard Model predictions are found. Exclusion limits are set on the production cross-section times branching ratio for hypothetical $Z'$ bosons, Kaluza-Kein gluons and Kaluza-Klein gravitons that decay into top-quark pairs.

==> EXOT-2015-04-PAPER-auxmat.tex <==
%\section{Auxiliary material}
\label{sec:appauxmat}

\begin{figure}[htbp]

\centering{
\subfigure[$Z' \rightarrow t\bar{t}$, boosted selection]{\includegraphics[width=0.45\textwidth]{auxmat/figures/accept/acceptboostedZp_ATLASSimul}}
\subfigure[$Z' \rightarrow t\bar{t}$, resolved selection]{\includegraphics[width=0.45\textwidth]{auxmat/figures/accept/acceptresolvedZp_ATLASSimul}}
\subfigure[$g_{KK} \rightarrow t\bar{t}$, boosted selection]{\includegraphics[width=0.45\textwidth]{auxmat/figures/accept/acceptboostedKKgluon_ATLASSimul}}
\subfigure[$g_{KK} \rightarrow t\bar{t}$, resolved selection]{\includegraphics[width=0.45\textwidth]{auxmat/figures/accept/acceptresolvedKKgluon_ATLASSimul}}
\subfigure[$G_{KK} \rightarrow t\bar{t}$, boosted selection]{\includegraphics[width=0.45\textwidth]{auxmat/figures/accept/acceptboostedKKgrav_ATLASSimul}}
\subfigure[$G_{KK} \rightarrow t\bar{t}$, resolved selection]{\includegraphics[width=0.45\textwidth]{auxmat/figures/accept/acceptresolvedKKgrav_ATLASSimul}}
}
\caption{Acceptance times selection efficiency, including branching ratio, 
as a function of the \ttbar quark invariant mass $m_{t\bar{t}}$ (computed after radiation but immediately before top quark decay) for simulated signal events. The dashed lines show the $\mu$+jets selection and the solid line shows the $e$+jets selection. 
\label{fig:BSMSelectionEff}}
\end{figure}

\begin{figure}[ht]
\centering
\subfigure[$m_{g_{\text{KK}}}=0.5$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg500unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\subfigure[$m_{g_{\text{KK}}}=1.5$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg1500unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\subfigure[$m_{g_{\text{KK}}}=2.0$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg2000unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\subfigure[$m_{g_{\text{KK}}}=2.5$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg2500unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\caption{The observed and expected cross-section 95\% CL upper limits on the $g_{\text{KK}}$ signal as a function of the resonance width for masses of (a) 0.5~\TeV{}, (b) 1.5~\TeV{},  (c) 2.0~\TeV{}, and  (d) 2.5~\TeV.}
\label{fig:limitvwidth_1}
\end{figure}

\begin{figure}[ht]
\centering
\subfigure[$m_{g_{\text{KK}}}=3.0$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg3000unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\subfigure[$m_{g_{\text{KK}}}=3.5$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg3500unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\subfigure[$m_{g_{\text{KK}}}=4.0$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg4000unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\subfigure[$m_{g_{\text{KK}}}=4.5$~\TeV{}]{\includegraphics[width=0.45\linewidth]{auxmat/figures/limits/final/unblinded/mass_limit_width_kkg4500unblind3_boottnorm_smooth2nnlottpspp8mbinsqcdfixzero3_dectau32_topptnnlo_ATLAS}}
\caption{The observed and expected cross-section 95\% CL upper limits on the $g_{\text{KK}}$ signal as a function of the resonance width for masses of (a) 3.0~\TeV{}, (b) 3.5~\TeV{},  (c) 4.0~\TeV{}, and  (d) 4.5~\TeV{}.}
\label{fig:limitvwidth_2}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{auxmat/figures/limits/final/unblinded/Ranking_zprime3tev_qcdfixzero3_ATLAS}
\caption{Effect of the nuisance parameter variations before and after the fit is performed on the 3~\TeV\ $Z^\prime_{\text{TC2}}$ model with a 1~pb signal cross-section.}
\label{fig:ranking_zprime3tev}
\end{figure}



==> tables_qcdfixzero3/yields_preFit.tex <==
\begin{tabular}{c|r@{$\pm$}l|r@{$\pm$}l|r@{$\pm$}l|r@{$\pm$}l}
\hline
\hline
&\multicolumn{8}{c}{Yields} \\
Type       & \multicolumn{2}{c}{Boosted e}  & \multicolumn{2}{c}{Boosted $\mu$} & \multicolumn{2}{c}{Resolved e} & \multicolumn{2}{c}{Resolved $\mu$} \\
\hline
  $t\overline{t}$    & \num[round-mode=figures,round-precision=3]{32277.94} & \num[round-mode=figures,round-precision=3]{2907.47101408} & \num[round-mode=figures,round-precision=3]{29428.45} & \num[round-mode=figures,round-precision=3]{2807.36434454} & \num[round-mode=figures,round-precision=3]{215124.0} & \num[round-mode=figures,round-precision=3]{16416.7383867} & \num[round-mode=figures,round-precision=3]{208572.6} & \num[round-mode=figures,round-precision=3]{16018.0163343} \\
  W+jets    & \num[round-mode=figures,round-precision=3]{2023.2436} & \num[round-mode=figures,round-precision=3]{311.591966851} & \num[round-mode=figures,round-precision=3]{2130.5124} & \num[round-mode=figures,round-precision=3]{281.680673041} & \num[round-mode=figures,round-precision=3]{8879.443} & \num[round-mode=figures,round-precision=3]{1538.13242804} & \num[round-mode=figures,round-precision=3]{9980.475} & \num[round-mode=figures,round-precision=3]{1168.00145453} \\
  multi-jet    & \num[round-mode=figures,round-precision=3]{3301.225} & \num[round-mode=figures,round-precision=3]{1161.07009915} & \num[round-mode=figures,round-precision=3]{1123.56} & \num[round-mode=figures,round-precision=3]{352.362776856} & \num[round-mode=figures,round-precision=3]{21901.72} & \num[round-mode=figures,round-precision=3]{8114.85225458} & \num[round-mode=figures,round-precision=3]{9761.42} & \num[round-mode=figures,round-precision=3]{3154.34095541} \\
  others    & \num[round-mode=figures,round-precision=3]{2737.117} & \num[round-mode=figures,round-precision=3]{282.240569524} & \num[round-mode=figures,round-precision=3]{2311.883} & \num[round-mode=figures,round-precision=3]{222.213708399} & \num[round-mode=figures,round-precision=3]{12098.43} & \num[round-mode=figures,round-precision=3]{1107.21292295} & \num[round-mode=figures,round-precision=3]{10425.17} & \num[round-mode=figures,round-precision=3]{930.720180521} \\
  Signal    & \num[round-mode=figures,round-precision=3]{987.87} & \num[round-mode=figures,round-precision=3]{48.5003787966} & \num[round-mode=figures,round-precision=3]{922.621} & \num[round-mode=figures,round-precision=3]{45.1624884216} & \num[round-mode=figures,round-precision=3]{276.9903} & \num[round-mode=figures,round-precision=3]{17.055694734} & \num[round-mode=figures,round-precision=3]{276.238} & \num[round-mode=figures,round-precision=3]{16.8851348883} \\
  Total    & \num[round-mode=figures,round-precision=3]{40339.5} & \num[round-mode=figures,round-precision=3]{3276.17712282} & \num[round-mode=figures,round-precision=3]{34994.5} & \num[round-mode=figures,round-precision=3]{2959.44133427} & \num[round-mode=figures,round-precision=3]{258004.1} & \num[round-mode=figures,round-precision=3]{19321.5688281} & \num[round-mode=figures,round-precision=3]{238739.6} & \num[round-mode=figures,round-precision=3]{17102.1987957} \\
\hline
  Data     & \multicolumn{2}{c}{35612.0}                                     & \multicolumn{2}{c}{31188.0}                                     & \multicolumn{2}{c}{261554.0}                                    & \multicolumn{2}{c}{254277.0}                                    \\
\hline
\hline
\end{tabular}

